A Grammar of Hypotheses for Visualization, Data, and Analysis

We present a grammar for expressing hypotheses in visual data analysis to formalize the previously abstract notion of "analysis tasks." Through the lens of our grammar, we lay the groundwork for how a user's data analysis questions can be operationalized and automated as a set of hypotheses (a hypothesis space). We demonstrate that our grammar-based approach for analysis tasks can provide a systematic method towards unifying three disparate spaces in visualization research: the hypotheses a dataset can express (a data hypothesis space), the hypotheses a user would like to refine or verify through analysis (an analysis hypothesis space), and the hypotheses a visualization design is capable of supporting (a visualization hypothesis space). We illustrate how the formalization of these three spaces can inform future research in visualization evaluation, knowledge elicitation, analytic provenance, and visualization recommendation by using a shared language for hypotheses. Finally, we compare our proposed grammar-based approach with existing visual analysis models and discuss the potential of a new hypothesis-driven theory of visual analytics.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> tabulars/low-lvl-tasks.tex <==

% \newcolumntype{b}{X}
% \newcolumntype{m}{>{\hsize=.45\hsize}X}
% \newcolumntype{s}{>{\hsize=.2\hsize}X}
\definecolor{palesilver}{rgb}{0.9, 0.9, 0.9}

\definecolor{palepink}{rgb}{0.98, 0.71, 0.68}
\definecolor{paleblue}{rgb}{0.7, 0.8, 0.89}
\definecolor{palegreen}{rgb}{0.8, 0.92, 0.77}
\definecolor{palepurp}{rgb}{0.87, 0.79, 0.89}

% \renewcommand\theadalign{bt}
% \renewcommand\theadfont{\bfseries}
% \renewcommand\theadgape{\Gape[4pt]}
% \renewcommand\cellgape{\Gape[4pt]}

% rgb(220,220,220)

% \resizebox{\textwidth}{!}{
% \begin{tabular}{p{0.15\linewidth} p{0.8\linewidth}}
% \begin{tabular}{ l l l }
% \toprule

% \textbf{Task} & 
% \textbf{Examples} &
% \textbf{Grammar} \\

% \hline

% Retrieve Value & Example & Grammar \\


% \hline 

% \end{tabular} %}
\renewcommand{\cellalign}{cl}

\begin{tabular}{p{0.2\linewidth} p{0.4\linewidth} p{0.35\linewidth}}
    \toprule
    
    \textbf{Task} & 
    \textbf{Example} &
    \textbf{Grammar} \\
    \hline
    % Retrieve Value
    % Retrieve Value & 
    %                     % question
    %                     What is the mileage per gallon of the Audi TT? &
    %                     % grammar
    %                     \begin{minipage}[l]{.35\textwidth}
    %                         \raggedleft
    %                         \begin{verbatim}
    %                         hello
    %                         \end{verbatim}
    %                     \end{minipage}
    %                     \\\hline
    
    % \multirow{2}{*}{Retrieve Value} & 
    %                     % question
    %                     \multicolumn{1}{l}{What is the mileage per gallon of the Audi TT?} &
    %                     % grammar
    %                     \multicolumn{1}{l}
    %                     {\texttt{hyp   :- ``MPG'' = const [Name=``Audi TT'']}} \\ &
    %                     % question
    %                     &
    %                     % grammar
    %                     \multicolumn{1}{l}
    %                     {\texttt{const :- number}} \\\hline
    
    Retrieve Value &
                    % question
                    What is the mileage per gallon of the Audi TT? &
                    % grammar
                    \makecell{
                        \texttt{hyp   :- ``MPG'' = const [pred]} \\
                        \texttt{pred  :- ``Name''=``Audi TT''} \\ 
                        \texttt{const :- number}
                    } \\ \hline 
    
    Filter & 
            % question
            What comedies have won awards? & 
            % grammar 
            \makecell{
                \texttt{hyp   :- ``Awards-won'' > 0 [pred]} \\
                \texttt{pred  :- ``Genre''=``Comedy''} \\ 
            } \\ \hline 
            % `Comedy1 has won an award''
                         
    
    Compute Derived Value &
            % question
            What is the average calorie content of Post cereals? &
            % grammar
            \makecell{
                \texttt{hyp   :- expr = const [pred] } \\
                \texttt{expr  :- func(``Calories'') } \\
                \texttt{func  :- AVG } \\
                \texttt{pred  :- Mfr=``Post''} \\ 
                \texttt{const :- number } \\ 
            } \\ \hline              
                         
    % Find Extremum
    Find Extremum & 
                        % question
                        What director/film has won the most awards? &
                        % grammar
                        \makecell{
                            \texttt{hyp   :- expr1 = expr2 [pred]}\\
                            \texttt{expr1  :- count () ``Awards-won'' } \\
                            \texttt{expr2  :- MAX(``Awards-won'') } \\
                            \texttt{pred  :- attr=``?'' }\\
                            \texttt{attr  :- ``Director'' | ``Film'' } \\ 
                        } \\ \hline  
                        % question
                        % Shawshank has won the most awards
                        % Christopher Nolan has won the most awards
                        % \multicolumn{1}{l}{ What Robin Williams film has the most recent release date?} &
                         
    % Sort
    Sort & 
                        % question
                        Order the cars by weight. &
                        % grammar
                        \makecell{
                            \texttt{hyp   :- expr1 > expr2 (\& hyp?) }\\
                            \texttt{expr1 :- ``Weight'' [``Name''=``?''] } \\
                            \texttt{expr2 :- ``Weight'' [``Name''=``?'']) } \\
                        } \\ \hline  
                        % question
                        % \multicolumn{1}{l}{Rank the cereals by calories.} &
                         
    % Determine Range
    Determine Range & 
                        % question
                        What is the range of film lengths? &
                        % grammar
                        \makecell{
                            \texttt{hyp   :- expr1 = const \& (expr2 = const) }\\
                            \texttt{expr1 :- MIN(``Duration'') } \\
                            \texttt{expr2 :- MAX(``Duration'') } \\
                            \texttt{const :- number } \\ 
                        } \\ \hline  
                        % question
                        % \multicolumn{1}{l}{What actresses are in the data set?} &
                         
    % Characterize Distribution
    \makecell{Characterize \\Distribution} & 
                        % question
                        What is the age distribution of shoppers? &
                        % grammar
                        \makecell{
                            \texttt{hyp       :- fit(``Age'', func) < const }\\
                            \texttt{func      :- Gaussian | Logarithmic | ... } \\
                            \texttt{const :- number } \\ 
                        } \\ \hline  
                        % question
                        % \multicolumn{1}{l}{ What is the age distribution of shoppers?} &
                         
    % Find Anomalies
    Find Anomalies & 
                        % question
                        Are there any outliers in protein? & 
                        % grammar
                        Grammar \\\hline
                        % question
                        % \multicolumn{1}{l}{Are there exceptions to the relationship between horsepower and acceleration? } &
                         
    % Cluster
    Cluster & 
                        % question
                        Are there groups of cereals with similar fat, calories, or sugar? &
                        % grammar
                        Grammar \\\hline
                        % question
                        % \multicolumn{1}{l}{Is there a cluster of typical film lengths?} &
                         
    % Correlate
    Correlate & 
                        % question
                        Is there a correlation between carbohydrates and fat? &
                        % grammar
                        Grammar \\\hline
                        % question
                        % \multicolumn{1}{l}{Is there a trend of increasing film length over the years?} &
                         
                         
    % Open-ended
    High-level & 
                        % question
                        Do any variables correlate with fat? &
                        % grammar
                        Grammar \\\hline
                        
    % uncertain criteria
    Uncertain criteria & 
                        % question
                        What other cereals are most similar to Trix? &
                        % grammar
                        Grammar \\\hline
                        % Compare the distributions of values for sugar and fat in the cereals
    
\end{tabular}

==> tabulars/old-low-lvl-tasks.tex <==

% \newcolumntype{b}{X}
% \newcolumntype{m}{>{\hsize=.45\hsize}X}
% \newcolumntype{s}{>{\hsize=.2\hsize}X}
\definecolor{palesilver}{rgb}{0.9, 0.9, 0.9}

\definecolor{palepink}{rgb}{0.98, 0.71, 0.68}
\definecolor{paleblue}{rgb}{0.7, 0.8, 0.89}
\definecolor{palegreen}{rgb}{0.8, 0.92, 0.77}
\definecolor{palepurp}{rgb}{0.87, 0.79, 0.89}

% \renewcommand\theadalign{bt}
% \renewcommand\theadfont{\bfseries}
% \renewcommand\theadgape{\Gape[4pt]}
% \renewcommand\cellgape{\Gape[4pt]}

% rgb(220,220,220)

% \resizebox{\textwidth}{!}{
% \begin{tabular}{p{0.15\linewidth} p{0.8\linewidth}}
% \begin{tabular}{ l l l }
% \toprule

% \textbf{Task} & 
% \textbf{Examples} &
% \textbf{Grammar} \\

% \hline

% Retrieve Value & Example & Grammar \\


% \hline 

% \end{tabular} %}

\begin{tabular}{p{0.2\linewidth} p{0.3\linewidth} p{0.3\linewidth}}
    \toprule
    
    \textbf{Task} & 
    \textbf{Examples} &
    \textbf{Grammar} \\
    \hline
    % Retrieve Value
    \multirow{2}{*}{Retrieve Value} & 
                        % question
                        \multicolumn{1}{l}{What is the mileage per gallon of the Audi TT?} &
                        % grammar
                        \multicolumn{1}{l}{XXX} \\\cline{2-3} &
                        % question
                        \multicolumn{1}{l}{How long is the movie Gone with the Wind?} &
                        % grammar
                        \multicolumn{1}{l}{XXX} \\\hline
                         
    % Filter
    \multirow{2}{*}{Filter} & 
                        % question
                        \multicolumn{1}{l}{What is the mileage per gallon of the Audi TT?} &
                        % grammar
                        \multicolumn{1}{l}{XXX} \\\cline{2-3} &
                        % question
                        \multicolumn{1}{l}{How long is the movie Gone with the Wind?} &
                        % grammar
                        \multicolumn{1}{l}{XXX} \\\hline
                         
    % Compute Derived Value
    \multirow{2}{*}{Compute Derived Value} & 
                        % question
                        \multicolumn{1}{l}{What is the average calorie content of Post cereals?} &
                        % grammar
                        \multicolumn{1}{l}{XXX} \\\cline{2-3} &
                        % question
                        \multicolumn{1}{l}{ What is the gross income of all stores combined?} &
                        % grammar
                        \multicolumn{1}{l}{XXX} \\\hline
                         
                         
    % Find Extremum
    \multirow{2}{*}{Find Extremum} & 
                        % question
                        \multicolumn{1}{l}{What director/film has won the most awards?} &
                        % grammar
                        \multicolumn{1}{l}{XXX} \\\cline{2-3} &
                        % question
                        \multicolumn{1}{l}{ What Robin Williams film has the most recent release date?} &
                        % grammar
                        \multicolumn{1}{l}{XXX} \\\hline
                         
    % Sort
    \multirow{2}{*}{Sort} & 
                        % question
                        \multicolumn{1}{l}{Order the cars by weight.} &
                        % grammar
                        \multicolumn{1}{l}{XXX} \\\cline{2-3} &
                        % question
                        \multicolumn{1}{l}{Rank the cereals by calories.} &
                        % grammar
                        \multicolumn{1}{l}{XXX} \\\hline
                         
    % Determine Range
    \multirow{2}{*}{Determine Range} & 
                        % question
                        \multicolumn{1}{l}{What is the range of film lengths?} &
                        % grammar
                        \multicolumn{1}{l}{XXX} \\\cline{2-3} &
                        % question
                        \multicolumn{1}{l}{What actresses are in the data set?} &
                        % grammar
                        \multicolumn{1}{l}{XXX} \\\hline
                         
    % Characterize Distribution
    \multirow{2}{*}{Characterize Distribution} & 
                        % question
                        \multicolumn{1}{l}{What is the distribution of carbohydrates in cereals?} &
                        % grammar
                        \multicolumn{1}{l}{XXX} \\\cline{2-3} &
                        % question
                        \multicolumn{1}{l}{ What is the age distribution of shoppers?} &
                        % grammar
                        \multicolumn{1}{l}{XXX} \\\hline
                         
    % Find Anomalies
    \multirow{2}{*}{Find Anomalies} & 
                        % question
                        \multicolumn{1}{l}{Are there exceptions to the relationship between horsepower and acceleration? } &
                        % grammar
                        \multicolumn{1}{l}{XXX} \\\cline{2-3} &
                        % question
                        \multicolumn{1}{l}{Are there any outliers in protein?} &
                        % grammar
                        \multicolumn{1}{l}{XXX} \\\hline
                         
    % Cluster
    \multirow{2}{*}{Cluster} & 
                        % question
                        \multicolumn{1}{l}{Are there groups of cereals w/ similar fat/calories/sugar?} &
                        % grammar
                        \multicolumn{1}{l}{XXX} \\\cline{2-3} &
                        % question
                        \multicolumn{1}{l}{Is there a cluster of typical film lengths?} &
                        % grammar
                        \multicolumn{1}{l}{XXX} \\\hline
                         
    % Correlate
    \multirow{2}{*}{Correlate} & 
                        % question
                        \multicolumn{1}{l}{Is there a correlation between carbohydrates and fat?} &
                        % grammar
                        \multicolumn{1}{l}{XXX} \\\cline{2-3} &
                        % question
                        \multicolumn{1}{l}{Is there a trend of increasing film length over the years?} &
                        % grammar
                        \multicolumn{1}{l}{XXX} \\\hline
                         
                         
    % Open-ended
    \multirow{2}{*}{High-level} & 
                        % question
                        \multicolumn{1}{l}{Do any variables correlate with fat?} &
                        % grammar
                        \multicolumn{1}{l}{XXX} \\\cline{2-3} &
                        % question
                        \multicolumn{1}{l}{How do mutual funds get rated?} &
                        % grammar
                        \multicolumn{1}{l}{XXX} \\\hline
    
\end{tabular}

==> tabulars/vast.tex <==

% \newcolumntype{b}{X}
% \newcolumntype{m}{>{\hsize=.45\hsize}X}
% \newcolumntype{s}{>{\hsize=.2\hsize}X}
\definecolor{palesilver}{rgb}{0.9, 0.9, 0.9}

\definecolor{palepink}{rgb}{0.98, 0.71, 0.68}
\definecolor{paleblue}{rgb}{0.7, 0.8, 0.89}
\definecolor{palegreen}{rgb}{0.8, 0.92, 0.77}
\definecolor{palepurp}{rgb}{0.87, 0.79, 0.89}

% \renewcommand\theadalign{bt}
% \renewcommand\theadfont{\bfseries}
% \renewcommand\theadgape{\Gape[4pt]}
% \renewcommand\cellgape{\Gape[4pt]}

% rgb(220,220,220)

% \resizebox{\textwidth}{!}{
\begin{tabular}{p{0.15\linewidth} p{0.8\linewidth}}
\toprule

\textbf{Question} & 
\textbf{Description} \\

\hline

% \rowcolor{palepink}
VAST 2017 MC1 Q1 & Describe daily patterns life by vehicles traveling through and within the park. Characterize the patterns by the kinds of vehicles participating, their spatial activities (where do they go?), and their temporal activities (when does the pattern happen?). \\

\hline

% \rowcolor{paleblue}
VAST 2017 MC1 Q2 & Describe patterns life that occur over multiple days by vehicles traveling through and within the park. Characterize the patterns by the kinds of vehicles participating, their spatial activities (where do they go?), and their temporal activities (when does the pattern happen?). \\

\hline
% \rowcolor{palegreen}
% VAST 2017 MC1 Q3 & Unusual patterns may be patterns of activity that changes from an established pattern, or are just difficult to explain from what you know of a situation. Describe up to six unusual patterns (either single day or multiple days) and highlight why you find them unusual. \\
VAST 2017 MC1 Q3 & Describe unusual patterns (either single day or multiple days) and highlight why you find them unusual. Unusual patterns may be patterns of activity that changes from an established pattern, or are just difficult to explain from what you know of a situation. \\

\hline 

\end{tabular} %}
